Corrected Block Sparse Spectral Optimization: Exact Models, Finite Identification, and Local Dynamics

The block generalized-power method pairs threshold-based support selection with inexpensive Stiefel updates, but the standard block formulation conflates two nonequivalent objectives and leaves inactive components, threshold ties, and post-selection refitting ill-specified. We rebuild the model from the primal. Eliminating each loading column from the normalized loading-ball problem gives a sum of soft-thresholded Euclidean norms (A-SUM); the squared-threshold objective in common use arises from a quadratic lift (A-SQ). We prove both identities, exhibit a two-component instance whose maximizers disagree, and specify explicit conventions for zero-response columns, ties, rank deficiency, and mask-before-refit. For A-SQ we separate the historical full-polar iteration from a safeguarded Riemannian ascent and prove, for the latter, whole-sequence convergence via a sufficient-ascent lemma, a relative-error lemma, and the Kurdyka-Lojasiewicz property, which applies because the soft-threshold objective and the Stiefel constraint are semi-algebraic. A strict threshold margin then forces finite identification of the support and sign pattern. The post-identification map is ordinary power iteration on the active covariance for a rank-one hard threshold, and the Frechet derivative of a coupled polar map for component-specific supports; a radius-based safe-screening rule follows from the same local analysis. Planted-spike experiments match the predicted identification time and local rates. On modern-AI panels (GPT-2 residual stream, ViT CLS stream, Pitprops) the thresholded block-sparse components match dense PCA on reconstruction and improve on it in monosemanticity and class specialisation. On three native-label scRNA datasets (Zheng17 FACS-sorted PBMCs, 68k donor-A with FACS-correlated labels, Tabula Muris) A-SQ beats dense PCA on cluster-recovery AMI by +0.023 to +0.044 at matched sparsity.

==> shared/brand/colors.tex <==
% SAIM semantic color system - single source of truth.
% Load xcolor before inputting this file.

% Core brand colors derived from the supplied SAIM identity.
\definecolor{SAIMIndigo}{HTML}{32127A}
\definecolor{SAIMIndigoDark}{HTML}{1A0A40}
\definecolor{SAIMLavender}{HTML}{D6CFE4}
\definecolor{SAIMLavenderLight}{HTML}{F5F2FA}
\definecolor{SAIMInk}{HTML}{17131F}
\definecolor{SAIMDark}{HTML}{211934}
\definecolor{SAIMCoolGray}{HTML}{F4F2F8}
\definecolor{SAIMPanel}{HTML}{FAF9FC}
\definecolor{SAIMMuted}{HTML}{6F6879}
\definecolor{SAIMRule}{HTML}{D8D3E1}
\definecolor{SAIMRuleDark}{HTML}{978EA7}
\definecolor{SAIMBlue}{HTML}{2E5C8A}
\definecolor{SAIMBluePale}{HTML}{EAF2F8}
\definecolor{SAIMGreen}{HTML}{4A7A5C}
\definecolor{SAIMGreenPale}{HTML}{EAF3ED}
\definecolor{SAIMRed}{HTML}{A74455}
\definecolor{SAIMRedPale}{HTML}{F8EAEE}
\definecolor{SAIMAmber}{HTML}{9B6418}
\definecolor{SAIMAmberPale}{HTML}{FFF4DD}

% Semantic names shared by the paper, slides, lecture notes, book, and gallery.
% White remains the default page and component interior; lavender is reserved
% for selected emphasis, diagrams, and optional soft backgrounds.
\colorlet{Primary}{SAIMIndigo}
\colorlet{PrimaryDark}{SAIMIndigoDark}
\colorlet{PrimaryPale}{white}
\colorlet{PrimaryWash}{white}
\colorlet{Secondary}{SAIMBlue}
\colorlet{SecondaryPale}{SAIMBluePale}
\colorlet{Positive}{SAIMGreen}
\colorlet{PositivePale}{SAIMGreenPale}
\colorlet{Negative}{SAIMRed}
\colorlet{NegativePale}{SAIMRedPale}
\colorlet{Warning}{SAIMAmber}
\colorlet{WarningPale}{SAIMAmberPale}
\colorlet{Ink}{SAIMInk}
\colorlet{Muted}{SAIMMuted}
\colorlet{Rule}{SAIMRule}
\colorlet{RuleDark}{SAIMRuleDark}
\colorlet{CodeBackground}{SAIMCoolGray}
\colorlet{LightPanel}{SAIMPanel}

% Compatibility aliases retained from the supplied SAIM templates.
\colorlet{saimindigo}{Primary}
\colorlet{saimbg}{SAIMLavender}
\colorlet{saimfg}{Ink}
\colorlet{saimdark}{SAIMDark}
\colorlet{saimgray}{SAIMCoolGray}
\colorlet{saimblue}{Secondary}
\colorlet{saimgreen}{Positive}
\colorlet{saimlight}{SAIMLavenderLight}
\colorlet{lightblue}{SecondaryPale}
\colorlet{metablue}{Secondary}
\colorlet{metafg}{Ink}
\colorlet{metabg}{LightPanel}


==> shared/brand/typography.tex <==
% SAIM Computer Modern Sans typography system - single source of truth.
% This reproduces the font system used by the reference Beamer deck:
% Computer Modern Sans for text, Computer Modern Typewriter for code, and the
% classic Computer Modern / AMS families for mathematics.
%
% The exact reference rendering is a pdfLaTeX system. No uploaded font files
% are required; all fonts ship with a standard TeX distribution.
\RequirePackage{fix-cm}
\RequirePackage[utf8]{inputenc}
\RequirePackage{textcomp}
\RequirePackage[protrusion=true,expansion=true]{microtype}
\RequirePackage{setspace}

% Use classic Computer Modern Sans everywhere ordinary text is requested.
% Mapping both Roman and Sans roles to cmss also converts legacy explicit
% \rmfamily calls in the template without creating a second visual family.
\renewcommand{\rmdefault}{cmss}
\renewcommand{\sfdefault}{cmss}
\renewcommand{\ttdefault}{cmtt}
\renewcommand{\familydefault}{\sfdefault}

% Computer Modern Sans provides a slanted face rather than a separate italic
% face. Route ordinary italic requests to that native slanted design so prose,
% citations, and code comments remain inside the reference font family.
\DeclareFontShape{OT1}{cmss}{m}{it}{<->ssub*cmss/m/sl}{}
\DeclareFontShape{OT1}{cmss}{bx}{it}{<->ssub*cmss/bx/n}{}
\normalfont

% Semantic font roles. All prose and display text share Computer Modern Sans;
% Mono marks technical literals. Mathematics remains the standard Computer
% Modern math system loaded by LaTeX and the AMS packages.
\providecommand{\SAIMBodyFont}{\sffamily}
\providecommand{\SAIMHeadingFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverTitleFont}{\sffamily\bfseries}
\providecommand{\SAIMCoverSubtitleFont}{\sffamily}
\providecommand{\SAIMNavigationFont}{\sffamily\bfseries}
\providecommand{\SAIMMetaFont}{\sffamily}
\providecommand{\SAIMCodeFont}{\ttfamily}

% Compatibility aliases used by the front-matter implementations.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/components/boxes.tex <==
% Shared tcolorbox vocabulary.
% Load tcolorbox with the `most` library before inputting this file.
\tcbset{
  saim/base/.style={
    enhanced,
    breakable,
    boxrule=0pt,
    arc=1.5pt,
    outer arc=1.5pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
    attach title to upper={\par\vspace{2pt}},
  },
  saim/primary/.style={
    saim/base,
    colback=PrimaryWash,
    borderline west={2.4pt}{0pt}{Primary},
    colframe=Primary,
  },
  saim/blue/.style={
    saim/base,
    colback=SecondaryPale,
    borderline west={2.4pt}{0pt}{Secondary},
    colframe=Secondary,
  },
  saim/green/.style={
    saim/base,
    colback=PositivePale,
    borderline west={2.4pt}{0pt}{Positive},
    colframe=Positive,
  },
  saim/amber/.style={
    saim/base,
    colback=WarningPale,
    borderline west={2.4pt}{0pt}{Warning},
    colframe=Warning,
  },
  saim/neutral/.style={
    saim/base,
    colback=LightPanel,
    borderline west={2.4pt}{0pt}{RuleDark},
    colframe=Rule,
  },
  saim/outline/.style={
    enhanced,
    breakable,
    colback=white,
    colframe=Rule,
    boxrule=0.55pt,
    arc=2pt,
    outer arc=2pt,
    left=8pt,
    right=8pt,
    top=7pt,
    bottom=7pt,
    before skip=8pt,
    after skip=8pt,
    fonttitle=\rmfamily\bfseries,
    coltitle=Ink,
  },
}


==> shared/components/evidence.tex <==
% Compact evidence-status labels usable in paper, slides, and book.
% Requires xcolor; no other package dependency.
\newcommand{\SAIMEvidenceTag}[3]{%
  \begingroup
  \setlength{\fboxsep}{2.6pt}%
  \setlength{\fboxrule}{0.45pt}%
  \raisebox{0.2ex}{\fcolorbox{#1}{#2}{%
    \textcolor{#1}{\sffamily\bfseries\fontsize{6.8}{8}\selectfont\textls[65]{\strut\MakeUppercase{#3}}}}}%
  \endgroup}
\newcommand{\MeasuredTag}{\SAIMEvidenceTag{Positive}{PositivePale}{Measured}}
\newcommand{\ReproducedTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{Reproduced}}
\newcommand{\SyntheticTag}{\SAIMEvidenceTag{Warning}{WarningPale}{Synthetic}}
\newcommand{\PlannedTag}{\SAIMEvidenceTag{RuleDark}{LightPanel}{Planned}}
\newcommand{\IllustrativeTag}{\SAIMEvidenceTag{PrimaryDark}{PrimaryWash}{Illustrative}}
\newcommand{\ExternalTag}{\SAIMEvidenceTag{Secondary}{SecondaryPale}{External}}


==> shared/components/frontmatter.tex <==
% Shared front-page typography roles.
% Computer Modern Sans is used consistently for title hierarchy, metadata,
% navigation, and prose, matching the reference Beamer deck.
\providecommand{\SAIMFrontFont}{\sffamily}
\providecommand{\SAIMFrontTitleFont}{\SAIMCoverTitleFont}
\providecommand{\SAIMFrontMetaFont}{\SAIMMetaFont}
\providecommand{\SAIMFrontRagged}{\raggedright\hyphenpenalty=10000\exhyphenpenalty=10000}


==> shared/components/listings.tex <==
% Shared code-listing styles. Load listings before inputting this file.
\lstdefinestyle{python}{
  language=Python,
  basicstyle=\ttfamily\small\color{Ink},
  keywordstyle=\color{PrimaryDark}\bfseries,
  stringstyle=\color{Positive},
  commentstyle=\color{Muted}\slshape,
  numberstyle=\scriptsize\color{RuleDark},
  numbers=left,
  numbersep=9pt,
  backgroundcolor=\color{CodeBackground},
  frame=leftline,
  rulecolor=\color{Primary},
  framerule=1.4pt,
  breaklines=true,
  showstringspaces=false,
  keepspaces=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}
\lstdefinestyle{console}{
  basicstyle=\ttfamily\small\color{Ink},
  backgroundcolor=\color{LightPanel},
  frame=leftline,
  rulecolor=\color{Secondary},
  framerule=1.4pt,
  breaklines=true,
  columns=fullflexible,
  xleftmargin=12pt,
  framexleftmargin=4pt,
  aboveskip=9pt,
  belowskip=9pt,
  captionpos=t,
}

